Investigating Positive and Negative Qualities of Human-in-the-Loop Optimization for Designing Interaction Techniques

Designers reportedly struggle with design optimization tasks where they are asked to find a combination of design parameters that maximizes a given set of objectives. In HCI, design optimization problems are often exceedingly complex, involving multiple objectives and expensive empirical evaluations. Model-based computational design algorithms assist designers by generating design examples during design, however they assume a model of the interaction domain. Black box methods for assistance, on the other hand, can work with any design problem. However, virtually all empirical studies of this human-in-the-loop approach have been carried out by either researchers or end-users. The question stands out if such methods can help designers in realistic tasks. In this paper, we study Bayesian optimization as an algorithmic method to guide the design optimization process. It operates by proposing to a designer which design candidate to try next, given previous observations. We report observations from a comparative study with 40 novice designers who were tasked to optimize a complex 3D touch interaction technique. The optimizer helped designers explore larger proportions of the design space and arrive at a better solution, however they reported lower agency and expressiveness. Designers guided by an optimizer reported lower mental effort but also felt less creative and less in charge of the progress. We conclude that human-in-the-loop optimization can support novice designers in cases where agency is not critical.

==> 2.current_practice.tex <==


THIS SECTION IS OBSOLETE = INTEGRATED TO SECTION 1


\section{Current practice of Design optimization in HCI} % Liwei

In this section, we briefly review empirical studies of design practice, focusing on the problems that designers face when optimizing designs. We then continue with a snapshot of academic papers in the CHI conference, reporting practices related to the optimization of technical parameters in interaction techniques.

\subsection{Design Practice}

Professional designers struggle with the challenge of generating high quality solutions in design \cite{cross2004expertise}. 
The current understanding is that they approach this challenge by two means: by refining objectives of the task, on the one hand, and taking different knowledge perspectives in order to generate candidate solutions, on the other \cite{dorst2001creativity,kruger2006solution}.
\emph{Goal refinement} refers to practices of elaborating a given task description. 
%Designers focus on goals and constraints in a problem statement and iteratively refine them.
When \emph{generating solutions}, designers shift between convergent and divergent thinking \cite{goldschmidt2016linkographic}.
These two concepts loosely map to exploitation and exploration in optimization literature, although convergent thinking is often associated with evaluative mindset \cite{goldschmidt2016linkographic}.
To generate solution candidates, designers use, among others, inspiring design examples, collaborative ideation methods, incubation strategies, and analogical thinking.

Empirical research has also exposed a number of \emph{biases} that limit the creative capability. A bias, here, means tendency to consider a skewed subsample in a design space. 
For example, confirmation bias occurs when designers collect evidence for an idea they like  \cite{hallihan2012confirmation}, 
anchoring bias occurs when we center our design solution around a known reference solution,  
decoying bias occurs when a reference point we have prevents us from seeing another one 'behind' it, and bandwagon bias occurs when we see peers following a solution. 
Generally, adherence to past ideas limits the creativity and quality of outcomes in design.
\emph{Fixation}, on the other hand, refers to 'blind adherence with a solution', or being unable or unwilling to generate an alternative \cite{jansson1991design}. 
%As a term, fixation is more constraining than biases: We are unable to let loose of a solution at hand and explore the space more broadly.
Designers may not even notice their fixation and, even expert designers, who are educated about fixations, exhibit fixation [ref].
Empirical literature suggests that fixations are hard to break \cite{agogue2014impact}. 
%After investing into producing a solution, the alternatives can perceived as riskier, less desirable, or involving too much effort. 
%However, seeing diverse design examples can help, assuming they are not \emph{too} divergent [ref]. To this end, designers are known to collect and curate example designs for this purpose [koch]. 
Computational methods could help break fixation by proposing task-relevant candidates [ref]. 

Designers employ a number of methods and processes that aim to address the limits posed by fixation and biases.
A shared feature of these is the rapid generation of lower-fidelity ideas early on in a project, most commonly by via sketching.
Rapid sketching, while keeping judgment at bay, avoids committing to a low-quality candidate too early in the process, 
and can help not only via the discovery of promising candidates but by recombining partial ideas from existing candidates \cite{verstijnen1998sketching}. 
%It is known that expert designers do more sketching, produce more ideas per unit of time, which on average are of higher quality [ref]. 
The takeaway for computational methods is that while they should support rapid exploration of ideas, they should not prevent adequate focus on promising candidates.

%The method we study in the rest of this paper offers a principled approach to avoid this.
%Computational support has little to say about goal refinement; it is normally assumed that input to the design algorithm is either precise or some sort of steering is allowed during the search the process \cite{oulasvirta2020combinatorial}.


\subsection{Optimization of Interaction Techniques in HCI Literature: A Snapshot from the CHI Conference}

To provide readers a glimpse of the current practices in HCI for optimizing interaction techniques, we discussed three interaction techniques designed for virtual reality published in CHI 2020. The three examples are meant to cover various types of practice HCI researchers or practitioners used in dealing with complex design problems involving multiple design parameters and objectives. Often, interaction technique research involves a stage of design optimization, be it with a pilot study or through a formal empirical setup, in which the aim is to determine parameter values that claim effective designs. In a separate empirical study, the effective designs are compared with other state-of-the-art baselines to claim effectiveness as the contribution. Specifically, we focused on how design optimization executed in these works manages design problems.

% removing parameters by referencing literature
HiveFive \cite{HiveFive} explored a visualization technique that aims to guide user attention in VR while preserving their immersion. The technique generated a localized swarm visual effect inserted into the scene. The design optimization is to have swarm motion seamlessly integrate as attentive directional cues into the scene without losing immersiveness. The formation of swarm motion involved four parameters that have a direct influence on the results, including the size of the bee and the number of bees in a swarm, and the velocity and spread of the swarm motion. The design objectives were ensuring visibility while avoiding clutter. Their optimization process involved first referencing the biology study of bee swarms to substantially narrow down the search range for each parameter, and second, fixing values in a pilot study (with three people). 

%Tackling parameters one-by-one
Body Follows Eye \cite{BodyFollowsEye} investigated an interaction technique that guides users’ posture change with them following a content window that is relocated each time the user blinks in VR. Design parameters of the technique were the detectable thresholds of window motions in translation and rotation. Because the thresholds would be varied by transition or rotation and by axis, this makes up a complex design problem involving six design parameters. The objectives were to increase window motions to effectively cause posture change while keeping the motion unnoticeable by the user. To keep the optimization manageable, they conducted a series of six sub-studies; each determined the threshold for one of the six motion types. However, the results were also limited to applying each time one motion type to the window.

% reducing points of evaluation
The ergonomic input technique \cite{ErgonomicsTouch} exploited applying the Hermite curve to amplify the user’s hand movements into a larger movement for increasing physical comfort while preserving ownership. The optimization of the interaction technique involved identifying four parameters that determine the mapping curve, with respect to the objectives of accuracy, comfort, and ownership. Finally, two configurations for the low and high amplification designs were concluded with a pilot with 5 users.

% \begin{enumerate}
% \item HiveFive: Immersion Preserving Attention Guidance in Virtual Reality, CHI 2020
% \begin{enumerate}
% \item Design Parameters (3): we found a velocity of 0.35m/second with a spread of 5 degrees visual angle in each direction most pleasant; We chose 10 bees to avoid cluttering
% \item Design Objectives (2): visibility, clutter
% \item Their solution: Fixed values in a pilot and by reference
% \end{enumerate}

% \item Body Follows Eye: Unobtrusive Posture Manipulation Through a Dynamic Content Position in Virtual Reality, CHI 2020
% \begin{enumerate}
% \item Design Parameters (6): speed of translations in 3 axis, speed of rotation in 3 axis; 2 directions * 5 steps per dimension
% \item Design Objectives (2): noticeable, time
% \item Their solution: tackles parameters one-by-one each with a formal study 
% \end{enumerate}

% \item Improving Reliability of Virtual Collision Responses: A Cue Integration Technique, CHI 2020
% \begin{enumerate}
% \item Design Parameters (4):  four parameters defined in Eq. 3 that determines movement speed of hand 
% \item Design Objectives (3): variance in direction, speed, diameter
% \item Their solution: formal study (16 participants)
% \end{enumerate}

% \item Improving Virtual Reality Ergonomics Through Reach-Bounded Non-Linear Input Amplification, CHI 2020
% \begin{enumerate}
% \item Design Parameters (2): Amplification (10)  x  Distance (3)
% \item Design Objectives (3): time, comfort, error
% \item Their solution: formal study (18 participants)
% \end{enumerate}
% \end{enumerate}



\subsection{summary}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX
